CLIP-DINOiser: Teaching CLIP a few DINO tricks for open-vocabulary semantic segmentation

The popular CLIP model displays impressive zero-shot capabilities thanks to its seamless interaction with arbitrary text prompts. However, its lack of spatial awareness makes it unsuitable for dense computer vision tasks, e.g., semantic segmentation, without an additional fine-tuning step that often uses annotations and can potentially suppress its original open-vocabulary properties. Meanwhile, self-supervised representation methods have demonstrated good localization properties without human-made annotations nor explicit supervision. In this work, we take the best of both worlds and propose an open-vocabulary semantic segmentation method, which does not require any annotations. We propose to locally improve dense MaskCLIP features, which are computed with a simple modification of CLIP's last pooling layer, by integrating localization priors extracted from self-supervised features. By doing so, we greatly improve the performance of MaskCLIP and produce smooth outputs. Moreover, we show that the used self-supervised feature properties can directly be learnt from CLIP features. Our method CLIP-DINOiser needs only a single forward pass of CLIP and two light convolutional layers at inference, no extra supervision nor extra memory and reaches state-of-the-art results on challenging and fine-grained benchmarks such as COCO, Pascal Context, Cityscapes and ADE20k. The code to reproduce our results is available at https://github.com/wysoczanska/clip_dinoiser.

==> figures/comparisons_correlations.tex <==
\begin{figure}
\centering
  \begin{subfigure}[b]{0.45\linewidth}
    \begin{tabular}{cc}
      \includegraphics[width=0.42\textwidth]{example-image}   &  \includegraphics[width=0.42\textwidth]{example-image}
    \end{tabular}
    \caption{\centering MaskCLIP corr.}
    \label{fig:corr-clip}
  \end{subfigure}
 \hfill
  \begin{subfigure}[b]{0.45\linewidth}
    \begin{tabular}{cc}
      \includegraphics[width=0.42\textwidth]{example-image}   &  \includegraphics[width=0.42\textwidth]{example-image}
    \end{tabular}
    \caption{DINO corr.}
    \label{fig:corr-dino}
  \end{subfigure}
 \hfill
  \begin{subfigure}[b]{0.45\linewidth}
    \begin{tabular}{cc}
      \includegraphics[width=0.42\textwidth]{example-image}   &  \includegraphics[width=0.42\textwidth]{example-image}
    \end{tabular}
    \caption{pred  corr.}
    \label{fig:corr-pred}
  \end{subfigure}
  \caption{\textbf{Comparison} of the patch correlation obtained with MaskCLIP features (a) and DINO self-supervised features (b) for different \emph{seed} patches noted in \textcolor{red}{red}.}
  \label{fig:corr-comparison}
\end{figure}

==> figures/main_pooling_res.tex <==
\newlength{\mainpoolingheight}
\setlength{\mainpoolingheight}{1.7cm}
\renewcommand{\arraystretch}{0.2}
% \begin{figure}[!ht]
% \centering
% \begin{subfigure}[b]{0.485\textwidth}
%     \centering
%     \includegraphics[width=.95\linewidth, trim={8em, 1.2em, 8em, 0}, clip] {figures/CLIPDINOiser_pooling.pdf}
%     \caption{\bf Our guided pooling.}
%     \label{fig:corr-zoom}
% \end{subfigure}
% % \hfill
% % \begin{subfigure}{.49\textwidth}
% %     \centering
% %     \setlength\tabcolsep{0.5pt}
% %     \begin{tabular}{cccc}
% %     ~ & \footnotesize{Context} & \footnotesize{ADE20K} & \footnotesize{CityScapes} \\
% %     \raisebox{+1.2\normalbaselineskip}[0pt][0pt]{\rotatebox[origin=c]{90}{\footnotesize{GT}}} & \includegraphics[height=\mainpoolingheight]{figures/ablations/ablation_gt.png} & 
% %     \includegraphics[height=\mainpoolingheight]{figures/ablations/ADE_val_00001221_overlay_gt.png} & 
% %     \includegraphics[height=\mainpoolingheight, trim={5em, 1.2em, 2em, 0}, clip]{figures/ablations/lindau_000008_000019_gtFine_overlay_gt.png}\\
% %     \raisebox{+1.2\normalbaselineskip}[0pt][0pt]{\rotatebox[origin=c]{90}{\footnotesize{using $F$}}}& \includegraphics[height=\mainpoolingheight]{figures/ablations/ablation_maskclip.png}& 
% %     \includegraphics[height=\mainpoolingheight]{figures/ablations/ADE_val_00001221_overlay_maskclip.png} & 
% %     \includegraphics[height=\mainpoolingheight, trim={5em, 1.2em, 2em, 0}, clip]{figures/ablations/lindau_000008_000019_gtFine_overlay_maskclip.png}\\
% %     %
% %     % \raisebox{+1.2\normalbaselineskip}[0pt][0pt]{\rotatebox[origin=c]{90}{\footnotesize{using $F^{+}$}}} & \includegraphics[height=\mainpoolingheight]{figures/ablations/ablation_ours.png} & 
% %     % \includegraphics[height=\mainpoolingheight]{figures/ablations/ADE_val_00001221_overlay_ours.png} & 
% %     % \includegraphics[height=\mainpoolingheight, trim={5em, 1.2em, 2em, 0}, clip]{figures/ablations/lindau_000008_000019_gtFine_overlay_ours.png}\\
% %     \end{tabular}
% %     \caption{\bf Impact of the pooling.}
% %     \label{fig:abl-maskclip}
% % \end{subfigure}
% \vspace{-10pt}
% \caption{\textbf{Guided pooling.} We present in (a) is our \emph{guided pooling} strategy defined in Eq.~\eqref{eq:refinement}.
% The $N\times N$ affinity matrix is computed from patch features and is used to refine MaskCLIP features (bottom left).
% % In (b) are the results after guided pooling (bottom) versus those obtained with original MaskCLIP features (middle).
% }
% \vspace{-10pt}
% % \end{figure*}
% \end{figure}

\begin{figure}[!h]
\centering
    \setlength\tabcolsep{0.5pt}
    \begin{tabular}{cccc}
    ~ & \footnotesize{Context} & \footnotesize{ADE20K} & \footnotesize{CityScapes} \\
    \raisebox{+1.2\normalbaselineskip}[0pt][0pt]{\rotatebox[origin=c]{90}{\footnotesize{GT}}} & \includegraphics[height=\mainpoolingheight]{figures/ablations/ablation_gt.png} & 
    \includegraphics[height=\mainpoolingheight]{figures/ablations/ADE_val_00001221_overlay_gt.png} & 
    \includegraphics[height=\mainpoolingheight, trim={5em, 1.2em, 2em, 0}, clip]{figures/ablations/lindau_000008_000019_gtFine_overlay_gt.png}\\
    \raisebox{+1.2\normalbaselineskip}[0pt][0pt]{\rotatebox[origin=c]{90}{\footnotesize{using $F$}}}& \includegraphics[height=\mainpoolingheight]{figures/ablations/ablation_maskclip.png}& 
    \includegraphics[height=\mainpoolingheight]{figures/ablations/ADE_val_00001221_overlay_maskclip.png} & 
    \includegraphics[height=\mainpoolingheight, trim={5em, 1.2em, 2em, 0}, clip]{figures/ablations/lindau_000008_000019_gtFine_overlay_maskclip.png}\\
    %
    % \raisebox{+1.2\normalbaselineskip}[0pt][0pt]{\rotatebox[origin=c]{90}{\footnotesize{using $F^{+}$}}} & \includegraphics[height=\mainpoolingheight]{figures/ablations/ablation_ours.png} & 
    % \includegraphics[height=\mainpoolingheight]{figures/ablations/ADE_val_00001221_overlay_ours.png} & 
    % \includegraphics[height=\mainpoolingheight, trim={5em, 1.2em, 2em, 0}, clip]{figures/ablations/lindau_000008_000019_gtFine_overlay_ours.png}\\
    \end{tabular}
\vspace{-10pt}
\caption{
% \textbf{Guided pooling} 
%We present in (a) is our \emph{guided pooling} 
% strategy defined in Eq.~\eqref{eq:refinement}.
% The $N\times N$ affinity matrix is computed from patch features and is used to refine MaskCLIP features (bottom left).
Results after guided pooling (bottom) versus those obtained with original MaskCLIP features (middle). \todo{return fig}
}
\vspace{-10pt}
% \end{figure*}
\end{figure}

==> figures/sup_bkg_qualitative.tex <==
\newlength{\pascalwidth}
\setlength{\pascalwidth}{0.17\textwidth}
\newlength{\cocowidth}
\setlength{\cocowidth}{0.12\textwidth}
\newlength{\citywidth}
\setlength{\citywidth}{0.20\textwidth}
\newlength{\resultsheight}
\setlength{\resultsheight}{1.6cm}

\newcommand{\addvoccocoresult}[3]{%
\begin{minipage}[b]{#1}
     \centering
     \includegraphics[width=\textwidth, height=\resultsheight]{figures/images/#2_#3.png}
\end{minipage}}
\newcommand{\addvoccocoresultjpeg}[2]{%
\begin{minipage}[b]{#1}
     \centering
     \includegraphics[width=\textwidth, height=\resultsheight]{figures/images/#2.jpg}
\end{minipage}}



\begin{figure*}[h]
\centering
\renewcommand{\arraystretch}{0}
\setlength\tabcolsep{0pt} 

% \rowcolors{7}{lightgray}{white}
\begin{center}
% \scalebox{0.95}
{
\begin{tabular}{
>{\centering\arraybackslash}m{7.5em} 
>{\centering\arraybackslash}m{\pascalwidth}
>{\centering\arraybackslash}m{\pascalwidth}
>{\centering\arraybackslash}m{\pascalwidth}
>{\centering\arraybackslash}m{\pascalwidth}
>{\centering\arraybackslash}m{\pascalwidth}
% ccccccc
}
\rule{0pt}{2.5ex} &  VOC & VOC & VOC & COCO & COCO \\
 {RGB} &
\addvoccocoresultjpeg{\pascalwidth}{2007_001834} & 
\addvoccocoresultjpeg{\pascalwidth}{2011_002410} &
\addvoccocoresultjpeg{\pascalwidth}{2007_002198} &
\addvoccocoresultjpeg{\pascalwidth}{000000074200} & 
\addvoccocoresultjpeg{\pascalwidth}{000000383386} \\

 {GT} &
\addvoccocoresult{\pascalwidth}{2007_001834}{gt} &
\addvoccocoresult{\pascalwidth}{2011_002410}{gt} &
\addvoccocoresult{\pascalwidth}{2007_002198}{gt} & 
\addvoccocoresult{\pascalwidth}{000000074200}{gt} &
\addvoccocoresult{\pascalwidth}{000000383386}{gt} \\

%%%%%%%% TCL

% \cline{1-2}
% \multirow{2}{*}[-1em]{\textsf{LL}$_3$ + \textsf{H3}} & 
 {TCL~\cite{cha2022tcl}}  &
\addvoccocoresult{\pascalwidth}{2007_001834}{tcl} &
\addvoccocoresult{\pascalwidth}{2011_002410}{tcl} &
\addvoccocoresult{\pascalwidth}{2007_002198}{tcl} & 
\addvoccocoresult{\pascalwidth}{000000074200}{tcl} & 
\addvoccocoresult{\pascalwidth}{000000383386}{tcl} \\

% \cline{1-2}
 {CLIP-DIY~\cite{wysoczanska2023clipdiy}} &
\addvoccocoresult{\pascalwidth}{2007_001834}{diy} &
\addvoccocoresult{\pascalwidth}{2011_002410}{diy} &
\addvoccocoresult{\pascalwidth}{2007_002198}{diy} & 
\addvoccocoresult{\pascalwidth}{000000074200}{diy} &
\addvoccocoresult{\pascalwidth}{000000383386}{diy} \\

\small{\ours} &
\addvoccocoresult{\pascalwidth}{2007_001834}{ours} &
\addvoccocoresult{\pascalwidth}{2011_002410}{ours} &
\addvoccocoresult{\pascalwidth}{2007_002198}{ours} & 
\addvoccocoresult{\pascalwidth}{000000074200}{ours} &
% \cocoresult{126216}{pred_final} &
\addvoccocoresult{\pascalwidth}{000000383386}{ours} \\

\vspace{1pt}
 % \global\let\CT@@do@color\relax % deactivate color
 Classes & 
 {\cellcolor[gray]{\graystrength} 
 \makecell{\promptstyle{diningtable}{dining table} \\ \promptstyle{chair_voc}{chair}}}
&
{\cellcolor[gray]{\graystrength} 
 \makecell{\promptstyle{car_voc}{car} }}
&
 {\cellcolor[gray]{\graystrength}\makecell
{\promptstyle{aeroplane_voc}{aeroplane} }}
&
{\cellcolor[gray]{\graystrength}\makecell 
{\promptstyle{surfboard_coco}{surfboard} \\ \promptstyle{potted plant_coco}{potted plant} \\
\promptstyle{snowboard_coco}{snowboard}}} 
& 
{\cellcolor[gray]{\graystrength}\makecell{
\promptstyle{teddy bear_coco}{teddy bear}  \\ \promptstyle{toilet_coco}{toilet} \\ \promptstyle{sports ball_coco}{sports ball}} }\\

\end{tabular}
}
\end{center}
    \vspace{-1.em}
    \caption{
    \textbf{Qualitative open-vocabulary segmentation results with `background' query}.
    }
    \label{fig:sup_bkg}
\end{figure*}

==> figures/sup_nobkg_qualitative.tex <==
\newlength{\pascalwidth}
\setlength{\pascalwidth}{0.165\textwidth}
\newlength{\cocowidth}
\setlength{\cocowidth}{0.12\textwidth}
\newlength{\citywidth}
\setlength{\citywidth}{0.20\textwidth}
\newlength{\resultsheight}
\setlength{\resultsheight}{1.7cm}

\newcommand{\addcocoablresulttwo}[3]{%
\begin{minipage}[b]{#1}
     \centering
     \includegraphics[width=\textwidth, height=\resultsheight]{figures/images/#2_#3.png}
\end{minipage}}
\newcommand{\addcocoablresulttwojpeg}[2]{%
\begin{minipage}[b]{#1}
     \centering
     \includegraphics[width=\textwidth, height=\resultsheight]{figures/images/#2.jpg}
\end{minipage}}



\begin{figure*}[ht]
\centering
\renewcommand{\arraystretch}{0}
\setlength\tabcolsep{0pt} 

% \rowcolors{7}{lightgray}{white}
\begin{center}
% \scalebox{0.95}
{

\begin{tabular}{
>{\centering\arraybackslash}m{7.5em} 
>{\centering\arraybackslash}m{\pascalwidth}
>{\centering\arraybackslash}m{\pascalwidth}
>{\centering\arraybackslash}m{\pascalwidth}
>{\centering\arraybackslash}m{\pascalwidth}
>{\centering\arraybackslash}m{\pascalwidth}
% ccccccc
}
\rule{0pt}{2.5ex} &  C59 & C59 & City & ADE20K & ADE20K \\
 {RGB} &
\addcocoablresulttwojpeg{\pascalwidth}{2009_003528} & 
\addcocoablresulttwojpeg{\pascalwidth}{2008_008546} &
\addcocoablresulttwo{\citywidth}{frankfurt_000001_047552}{} &
\addcocoablresulttwojpeg{\pascalwidth}{ADE_val_00001334} & 
\addcocoablresulttwojpeg{\pascalwidth}{ADE_val_00001623} \\

 {GT} &
\addcocoablresulttwo{\pascalwidth}{2009_003528}{gt} &
\addcocoablresulttwo{\pascalwidth}{2008_008546}{gt} &
\addcocoablresulttwo{\citywidth}{frankfurt_000001_047552}{gt} & 
\addcocoablresulttwo{\pascalwidth}{ADE_val_00001334}{gt} &
\addcocoablresulttwo{\pascalwidth}{ADE_val_00001623}{gt} \\

%%%%%%%% TCL

% \cline{1-2}
% \multirow{2}{*}[-1em]{\textsf{LL}$_3$ + \textsf{H3}} & 
 {TCL~\cite{cha2022tcl}}  &
\addcocoablresulttwo{\pascalwidth}{2009_003528}{tcl} &
\addcocoablresulttwo{\pascalwidth}{2008_008546}{tcl} &
\addcocoablresulttwo{\citywidth}{frankfurt_000001_047552}{tcl} & 
\addcocoablresulttwo{\pascalwidth}{ADE_val_00001334}{tcl} & 
\addcocoablresulttwo{\pascalwidth}{ADE_val_00001623}{tcl} \\

% \cline{1-2}
 {CLIP-DIY~\cite{wysoczanska2023clipdiy}} &
\addcocoablresulttwo{\pascalwidth}{2009_003528}{diy} &
\addcocoablresulttwo{\pascalwidth}{2008_008546}{diy} &
\addcocoablresulttwo{\citywidth}{frankfurt_000001_047552}{diy} & 
\addcocoablresulttwo{\pascalwidth}{ADE_val_00001334}{diy} &
\addcocoablresulttwo{\pascalwidth}{ADE_val_00001623}{diy} \\

\small{\ours} &
\addcocoablresulttwo{\pascalwidth}{2009_003528}{ours} &
\addcocoablresulttwo{\pascalwidth}{2008_008546}{ours} &
\addcocoablresulttwo{\citywidth}{frankfurt_000001_047552}{ours} & 
\addcocoablresulttwo{\pascalwidth}{ADE_val_00001334}{ours} &
% \cocoresult{126216}{pred_final} &
\addcocoablresulttwo{\pascalwidth}{ADE_val_00001623}{ours} \\

\small
\vspace{1pt}
 % \global\let\CT@@do@color\relax % deactivate color
 Classes & 
 {\cellcolor[gray]{\graystrength} 
 \makecell{\promptstyle{cat_context}{cat}  \promptstyle{sidewalk_context}{sidewalk} \\ \promptstyle{ground_context}{ground} \promptstyle{grass_context}{grass} \\ \promptstyle{floor_context}{floor}}}
&
{\cellcolor[gray]{\graystrength} 
 \makecell{\promptstyle{aeroplane_context}{aeroplane} \\
 \promptstyle{mountain_context}{mountain} \promptstyle{sky_context}{sky} \\ \promptstyle{cloth_context}{cloth}}}
&
{\cellcolor[gray]{\graystrength}\makecell
{\promptstyle{road_city}{road} \promptstyle{vegetation_city}{vegetation} \\
 \promptstyle{car_city}{car} \promptstyle{sidewalk_city}{sidewalk} \\ \promptstyle{person_city}{person} }}
&
{\cellcolor[gray]{\graystrength}\makecell 
{\promptstyle{road_ade}{road} \promptstyle{tree_ade}{tree} \\
\promptstyle{house_ade}{house} \promptstyle{palm_ade}{palm} \\ \promptstyle{sidewalk_ade}{sidewalk} \promptstyle{sky_ade}{sky}}} 
& 
{\cellcolor[gray]{\graystrength}\makecell{
\promptstyle{rock_ade}{rock} \promptstyle{sea_ade}{sea} \\ \promptstyle{sky_ade}{sky} \\ \promptstyle{light_ade}{light}} }\\

\end{tabular}
}
\end{center}
    \vspace{-1.em}
    \caption{
    \textbf{Qualitative open-vocabulary segmentation results}.
    }
    % \vspace{-0.5cm}
    \label{fig:sup_nobkg}
\end{figure*}

==> tables/main_res_bg_final.tex <==
\newcommand{\resultsrowbg}[8]{#1 & #2 & #3 & #4 & #5 & #6 & #7 & #8}

\begin{table}[ht]
\centering
\small
\renewcommand{\arraystretch}{1.0}
\setlength{\tabcolsep}{1pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|cccc|ccc}
\toprule
\toprule
\resultsrowbg{}
{Concept}
{Frozen}
{Extra}
{Backbone}
{}
{} 
{} 
\\
\resultsrowbg{\textbf{Methods}}
{spec.}
{back.}
{Data}
{at inference}
{Context}
{Object} 
{VOC} \\
\midrule
\rowcolor{Black!10!white} \multicolumn{8}{l}{\textcolor{Black!10!white}{aaaaaaa} \textbf{Dataset specific}} \\
\resultsrowbg{MaskCLIP+~\cite{zhou2022maskclip}}
{\checkmark}
{\xmark}
{Target}
{DeepLabv2}
{23.6} % Context
{20.6} % Object 
{38.8} % VOC

\\
\resultsrowbg{NamedMask~\cite{shin2023namedmask}}
{\checkmark}
{\xmark}
{IN(1.2M)+Target}
% {IN(1.2M im.)+Target dataset}
{DeepLabv3+}
{-} % Context
{27.7} % Object
{59.2} % VOC
\\

\midrule
% \multicolumn{7}{l}{---\emph{Builds prototypes per visual concept}---} 
\rowcolor{Black!10!white} \multicolumn{8}{l}{\textcolor{Black!10!white}{aaaaaaa} \textbf{Builds prototypes per visual concept}}
\\
\resultsrowbg{ReCo~\cite{shin2022reco}}
% {CLIP-ViT}
% {CLIP-Text}
{\checkmark}
{\xmark}
{IN(1.2M)}
{CLIP}
{19.9} % Context
{15.7} % Object 
{25.1} % VOC
\\

\resultsrowbg{OVDiff~\cite{karazija2023diffusion} }
{\checkmark}
{\checkmark}
{\xmark}
{CLIP+DINO+SD}
{\underline{30.1}} % Context
{\bf 34.8} % Object
{\bf 67.1} % VOC
\\

\midrule
\rowcolor{Black!10!white} \multicolumn{8}{l}{\textcolor{Black!10!white}{aaaaaaa} \textbf{Text/image alignment training w/ captions}} \\

\resultsrowbg{GroupViT~\cite{xu2022groupvit}}
{\xmark}
{\xmark}
% {TODO}
{CC12M+RedCaps}
{CLIP}
{18.7} % Context
{27.5} % Object 
{50.4} % VOC
\\

\resultsrowbg{ZeroSeg~\cite{Chen_2023_ICCV}}
{\xmark}
{\xmark}
{IN(1.2M)+CC12M}
{CLIP}
{21.8} % Context
{22.1} % Object 
{42.9} % VOC
\\

\resultsrowbg{SegCLIP~\cite{lou2022segclip}}
{\xmark}
{\xmark}
{CC3M+COCO}
{CLIP}
{24.7} % Context
{26.5} % Object 
{52.6} % VOC
\\

\resultsrowbg{TCL~\cite{cha2022tcl}}
{\xmark}
{\xmark}
{CC12M+CC3M}
{CLIP}
{24.3} % Context
{30.4} % Object 
{51.2} % VOC
\\

\resultsrowbg{CLIPpy~\cite{clippy2022}}
{\xmark}
{\xmark}
{HQITP-134M}
{CLIP}
{-} % Context
{32.0} % Object 
{52.2} % VOC
\\

\resultsrowbg{OVSegmentor~\cite{xu2023learning}}
{\xmark}
{\xmark}
{CC4M}
{CLIP}
{20.4} % Context
{25.1} % Object 
{53.8} % VOC
\\

\midrule
\midrule

\rowcolor{Black!10!white} \multicolumn{8}{l}{\textcolor{Black!10!white}{aaaaaaa} \textbf{Frozen CLIP}} \\

\resultsrowbg{CLIP-DIY~\cite{wysoczanska2023clipdiy}}
{\xmark}
{\checkmark}
{\xmark}
{CLIP+DINO}
{19.7} % Context
{31.0} % Object 
{59.9} % VOC
\\

\resultsrowbg{MaskCLIP~\cite{zhou2022maskclip}}
{\xmark}
{\checkmark}
{\xmark}
{CLIP}
{21.1} % Context
{15.5} % Object 
{29.3} % VOC
\\

\resultsrowbg{MaskCLIP$^*$}
{\xmark}
{\checkmark}
{\xmark}
{CLIP}
{22.9} % Context 
{16.4} % Object
{32.9} % VOC
\\


\resultsrowbg{MaskCLIP$^*$$\dag$}
{\xmark}
{\checkmark}
{\xmark}
{CLIP}
{24.0} % Context
{21.6} % Object
{41.3} % VOC
\\

\resultsrowbg{\rowcolor{ForestGreen!20!white} \ours}
{\xmark}
{\checkmark}
{IN (random 1k im.)}
{CLIP}
{\bf 32.4} % Context
{\bf 34.8} % Object
{\underline{62.1}} % VOC
\\

\bottomrule
\end{tabular}
}
\vspace{0.1cm}
\caption{
\textbf{Open-vocabulary semantic segmentation} evaluation on datasets \emph{with} `background'.
We report all methods without post-processing. 
We refer to \cref{table:main_nobg} for details about notations.
}
\label{table:main_bg}
\end{table}


==> tables/main_res_nobg_final.tex <==
\newcommand{\resultsrownobg}[9]{#1 & #2 & #3 & #4 & #5 & #6 & #7 & #8 & #9 & \more}
\newcommand{\more}[1]{#1}

\begin{table*}[ht]
\centering
\small
\renewcommand{\arraystretch}{1.0}
\setlength{\tabcolsep}{1pt}
% \resizebox{\linewidth}{!}{
\begin{tabular}
{l|cccc|ccccc}
\toprule
\toprule
\resultsrownobg
{}
{\textbf{Concept}}
{\textbf{Frozen}}
{\textbf{Extra}}
{\textbf{Backbone}}
{}
{}
{}
{}
{} \\
\resultsrownobg
{\textbf{Methods}}
{\textbf{spec.}}
{\textbf{backbone}}
{\textbf{data}}
{\textbf{at inference}}
{\textbf{VOC20}}
{\textbf{C59}}
{\textbf{Stuff}}
{\textbf{City}}
{\textbf{ADE}} \\

\midrule
\rowcolor{Black!10!white} \multicolumn{10}{l}{\textcolor{Black!10!white}{aaaaaaa} \textbf{Dataset specific}} \\
\resultsrownobg
{MaskCLIP+~\cite{zhou2022maskclip}}
{\checkmark}
{\xmark}
{Target dataset}% {Pseudo labels}
{DeepLabv2}
{74.9} % VOC20
{26.4} % Context59
{16.4} % Stuff
{9.8} % City
{10.8} \\ %ADE 

\midrule
\rowcolor{Black!10!white} \multicolumn{10}{l}{\textcolor{Black!10!white}{aaaaaaa} \textbf{Build prototypes per visual concept}} \\

\resultsrownobg
{ReCo~\cite{shin2022reco}}
{\checkmark}
{\checkmark}
{IN (1.2M im.)}
{CLIP}
{57.8} % VOC20
{22.3} % Context59
{14.8} % Stuff
{21.1} % City
{11.2} \\ %ADE 
% 23.5

\resultsrownobg
{OVDiff~\cite{karazija2023diffusion}}
{\checkmark}
{\checkmark}
{\xmark}
{CLIP+DINO+SD}
{\bf 81.7} % VOC20
{\underline{33.7}} % Context59
{-} % Stuff
{-} % City
{\underline{14.9}} \\ %ADE 

\midrule
\rowcolor{Black!10!white} \multicolumn{10}{l}{\textcolor{Black!10!white}{aaaaaaa} \textbf{Text/image alignment training with captions}} \\

\resultsrownobg
{GroupViT~\cite{xu2022groupvit}}
{\xmark}
{\xmark}
{CC12M+RedCaps}
{CLIP}
{79.7} % VOC20
{23.4} % Context59
{15.3} % Stuff
{11.1} % City
{9.2} \\ %ADE

\resultsrownobg
{SegCLIP~\cite{lou2022segclip}}
{\xmark}
{\xmark}
{CC3M+COCO(400k)}
{CLIP}
{-} % VOC20
{-} % Context59
{-} % Stuff
{11.0} % City
{8.7} \\ %ADE 

\resultsrownobg
{TCL~\cite{cha2022tcl}}
{\xmark}
{\xmark}
{CC12M+CC3M}
{CLIP}
{77.5} % VOC20
{30.3} % Context59
{\underline{19.6}} % Stuff
{23.1} % City
{\underline{14.9}} \\ %ADE 

\resultsrownobg
{CLIPpy~\cite{clippy2022}}
{\xmark}
{\xmark}
{HQITP-134M~\cite{clippy2022}}
{CLIP}
{-} % VOC20
{-} % Context59
{-} % Stuff
{-} % City
{13.5} \\ %ADE 

\resultsrownobg
{OVSegmentor~\cite{xu2023learning}}
{\xmark}
{\xmark}
{CC4M~\cite{xu2023learning}}
{CLIP}
{-} % VOC20
{-} % Context59
{-} % Stuff
{-} % City
{5.6} \\ %ADE 

\midrule
\midrule

\rowcolor{Black!10!white} \multicolumn{10}{l}{\textcolor{Black!10!white}{aaaaaaa} \textbf{Frozen CLIP}} \\

\resultsrownobg
{CLIP-DIY~\cite{wysoczanska2023clipdiy}$^{*}$}
{\xmark}
{\checkmark}
{\xmark}
{CLIP+DINO}
{79.7} % VOC20
{19.8} % Context59
{13.3} % Stuff
{11.6} % City
{9.9} \\ %ADE 

\resultsrownobg
{MaskCLIP~\cite{zhou2022maskclip}~\cite{cha2022tcl}}
{\xmark}
{\checkmark}
{\xmark}
{CLIP}
{53.7} % VOC20
{23.3} % Context59
{14.7} % Stuff
{21.6} % City
{10.8} \\ %ADE 

\resultsrownobg
{MaskCLIP$^{*}$} %(OpenCLIP Laion 2B)}
{\xmark}
{\checkmark}
{\xmark}
{CLIP}
{61.8} % VOC20
{25.6} % Context59
{17.6} % Stuff
{\underline{25.0}} % City
{14.3} \\ %ADE 

\resultsrownobg
{MaskCLIP$^{*}$ $\dag$} %(OpenCLIP Laion 2B)}
{\xmark}
{\checkmark}
{\xmark}
{CLIP}
{71.9} % VOC20
{27.4} % Context59
{18.6} % Stuff
{23.0} % City
{\underline{14.9}} \\ %ADE

\resultsrownobg
{\rowcolor{ForestGreen!15!white} \oursnormal}
{\xmark}
{\checkmark}
{IN (random 1k im.)}
% {\xmark}
{CLIP}
{\underline{80.9}} % VOC20
{\bf35.9} % Context59
{\bf24.6} % Stuff
{\bf31.7} % City
{\bf20.0} \\ %ADE 

\bottomrule
\end{tabular}
% }
\vspace{0.1cm}

\caption{\textbf{Open-vocabulary semantic segmentation quantitative comparison on datasets without `background'} class using the mIoU metric. 
We report all methods without post-processing. We note with $^*$ methods for which we computed scores; we obtained  MaskCLIP$^{*}$ scores with OpenCLIP~\cite{openclip}. 
We also mark with $\dag$ the use of MaskCLIP refinement. 
The first and second best methods are respectively \textbf{bold} and \underline{underlined}.
We include additional information on whether a model (1) assumes prior access to names of concepts (`Concept spec.'), (2) uses a frozen backbone (`Frozen backbone'), (3) employs training with additional data (`Extra data'), (4) and the kind of backbones used at inference time (`Backbone at inference'). `IN' stands for ImageNet \cite{imagenet} and `SD' for Stable Diffusion \cite{rombach2022high}.
We provide here the references for the image/text training dataset used by some methods: CC12M~\cite{changpinyo2021conceptual}, CC3M~\cite{cc2018}, RedCaps~\cite{desai2021redcaps} and COCO~\cite{lin2014microsoft}.
We refer to \cref{sec:setup} for more details on baselines.
}
\label{table:main_nobg}
\end{table*}



